Discontinuous Galerkin Methods for Mass Transfer through Semi-Permeable Membranes

A discontinuous Galerkin (dG) method for the numerical solution of initial/boundary value multi-compartment partial differential equation (PDE) models, interconnected with interface conditions, is presented and analysed. The study of interface problems is motivated by models of mass transfer of solutes through semi-permeable membranes. More specifically, a model problem consisting of a system of semilinear parabolic advection-diffusion-reaction partial differential equations in each compartment, equipped with respective initial and boundary conditions, is considered. Nonlinear interface conditions modelling selective permeability, congestion and partial reflection are applied to the compartment interfaces. An interior penalty dG method is presented for this problem and it is analysed in the space-discrete setting. The a priori analysis shows that the method yields optimal a priori bounds, provided the exact solution is sufficiently smooth. Numerical experiments indicate agreement with the theoretical bounds and highlight the stability of the numerical method in the advection-dominated regime.

==> numex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Numerical examples}\label{sec:numex}

In view of the numerical tests, we introduce a fully discrete discretisation
for the system (\ref{pde}), (\ref{modelbc}), (\ref{transmission}).
The time discretization is based on a second-order linearly implicit method 
analysed in~\cite{MR1701828,Crouzeix,Akrivis04}.
%, that is  we discretize the linear terms  and the nonlinear terms by, respectively, an implicit and explicit method, both second order accurate.

Let us write the semidiscrete DG formulation~\eqref{eq:semidiscrete} in matrix notation as
\begin{equation}\label{eq:algebric}
{\rm M \rm U_t = LU + F(U)}
\end{equation}
where ${\rm L}$ collects all linear terms and ${\rm F}$ the nonlinear terms in~\eqref{eq:semidiscrete}.
Treating the linear terms with the second-order Adams–Moulton method (trapezium rule) and the
nonlinear terms with the second-order Adams–Bashforth method  yields the following
fully discrete method (AB2-AM2):
\[
M U^{n+1}= MU^n + k (\theta A U^{n+1}+(1-\theta) A U^{n})+\frac{k}{2}(3 F(U^n)-F(U^{n-1})).
\]

{\bf Convergence test.} We test the validity of the IPDG method and above error bounds on a system of two equations for which the exact solution is known.

Let the domain $\Omega=[-1,1]^2$ be subdivided into two subdomains interfacing at $x=0$; thus
$\Omega^1=[-1,0]\times [-1,1]$ and $\Omega^2=[0,1]\times [-1,1]$.
We set $\Gamma_{\ddd}=\{ \pm1\}\times [-1,1]$ and 
$\Gamma_{\dn}=(-1,1)\times\{ \pm1\}$ and
impose homogeneous Dirichlet and Neumann boundary conditions
on $\Gamma_{\ddd}$ and $\Gamma_{\dn}$, respectively, as shown in Figure~\ref{fig:domain} (left).
\begin{figure}[!t]
\begin{center}
\setlength{\unitlength}{2cm}
\begin{picture}(0,0)
\put(0,0){\line(0,1){2}}
\put(1,0){\line(0,1){2}}
\put(0,0){\line(1,0){1}}
\put(0,1){\line(1,0){1}}
\put(0,2){\line(1,0){1}}
\put(.5,.5){\makebox(0,0){\tiny{$\Omega^1$}}}
\put(.5,1.5){\makebox(0,0){\tiny{$\Omega^2$}}}
\put(.7,1.06){\makebox(0,0){\tiny{{{$\Gatr$}}}}}
\put(.43,1.2){\makebox(0,0){\tiny{$x$}}}
\put(.3,1.1){\makebox(0,0){\tiny{$y$}}}
\put(-.12,1){\makebox(0,0){\rotatebox{90}{\tiny{$\frac{\partial \bu}{\partial\mbf{n}}=\mbf{0}$}}}}
\put(1.1,1){\makebox(0,0){\rotatebox{90}{\tiny{$\frac{\partial \bu}{\partial\mbf{n}}=\mbf{0}$}}}}
\put(.5,1){\vector(-1,0){.2}}
\put(.5,1){\vector(0,1){.2}}
\put(.5,-.1){\makebox(0,0){\tiny{$\bu=\mbf{0}$}}}
\put(.5,2.1){\makebox(0,0){\tiny{$\bu=\mbf{0}$}}}
\end{picture}
\hspace{25 mm}
\begin{overpic}[scale=0.4]{u1_541.pdf}
 \small{\put(80,3){$x$}
        \put(26,3){$y$}
        \put(4,37){$u_1$}
       }
\end{overpic}
\end{center}
\caption{Convergence test. Solution domain and boundary conditions (left). First component of the exact solution at
the final time $t=1$ (right).}
\label{fig:domain}
\end{figure}
For $t>0$ we consider the system of two advection-diffusion equations
\begin{equation}\label{ex2:system}
\left\{
\begin{array}{l}
\vspace{2 mm}
u_t - \Delta u -u_x   = f^u +
\left\{
\hspace{-2 mm}
\begin{array}{ll}
\vspace{1 mm}
  u^2 - v (1-v) &\T{in $\Omega^1$}\\
 - v &\T{in } \Omega^2,\\
\end{array}
\right.\\
v_t - \Delta v -v_x = f^v+u \quad\T{in $\Omega^1\cup \Omega^2$},
\end{array}
\right.
\end{equation}
and accordingly construct the forcing terms
$f^{u,v}:[0,1]\times\Omega\rightarrow\mathbb{R}$ in order to
yield as exact solution
\begin{equation}\label{ex2:solution}
\left(\hspace{-1 mm}
\begin{array}{c}
\vspace{1 mm}
u\\
v
\end{array}
\hspace{-1 mm}
\right)      =
\left(\hspace{-1 mm}
\begin{array}{c}
\vspace{1 mm}
\cos t\\
\sin t
\end{array}
\hspace{-1 mm}
\right)
e^{(y^2-1)^2}
\times
\left\{
\begin{array}{ll}
\vspace{1 mm}
4 x (1 + x)
 & \T{in $\Omega^1$,}\\
(- 4 x^3  + 3 x + 1) &\T{in $\Omega^2$}.
\end{array}
\right.
\end{equation}
The first component of the solution at 
time $t=1$ is shown in 
Figure~\ref{fig:domain} (right).
The functions in~\eqref{ex2:solution} are compatible
with the interface conditions~\eqref{transmission}
with respect to the interface parameters %constant and diagonal permeability tensor 
\[
\mbf{P}=\T{diag}(3,3), 
\qquad 
\Weight^{1} =\T{diag}(1,1),
\qquad 
\Weight^{2} =\T{diag}(0,0),
\qquad 
\Friction =\T{diag}(1,1),
\]
which are therefore used to close 
problem~\eqref{ex2:system} with 
conditions~\eqref{transmission}.
%friction $\friction_{1,2}=1$, and weights $%\weight_{1,2}^1=1$, $\weight_{1,2}^2=0$.

%We solve numerically problem~\eqref{ex2:system} using the fully discrete
%IPDG method described above 
We tested the convergence rate of our method
under space discretisation refinement.
A fixed time step of size $.5\times 10^{-3}$ is used throughout while an initial uniform square $4\times 4$ mesh is uniformly refined. The value $C_{\sigma}=10$ was used throughout for the discontinuity-penalization parameter costant.
Numerical results are reported in Table~\ref{table:ex2} in the cases of linear and quadratic spatial discretizations. 
The predicted error rates of convergenece are confirmed in  both the ${L^2(0,1;\SSpace)}$ and ${L^{\infty}(0,1;L^2(\Omega))}$ norms.
\begin{table}[!t]
    \label{table:ex2}
\begin{center}
\begin{tabular}{|r|r|c|c|c|c|} \hline
\# cells & \# dofs &
\multicolumn{2}{|c|}{${L^2(0,1;\SSpace)}$} &
\multicolumn{2}{|c|}{${L^{\infty}(0,1;L^2(\Omega))}$}\\ \hline
\multicolumn{6}{c}{${\tt m}\equiv 1$}\\ \hline
4 & 32 & 1.579e+01 & - & 2.498e+00 & -\\ \hline
16 & 128 & 7.617e+00 & 1.05 & 8.293e-01 & 1.59\\ \hline
64 & 512 & 3.615e+00 & 1.08 & 2.400e-01 & 1.79\\ \hline
256 & 2048 & 1.736e+00 & 1.06 & 6.497e-02 & 1.89\\ \hline
1024 & 8192 & 8.475e-01 & 1.03 & 1.693e-02 & 1.94\\ \hline
4096 & 32768 & 4.182e-01 & 1.02 & 4.324e-03 & 1.97\\ \hline
%\end{tabular}
%\begin{tabular}{|r|r|c|c|c|c|} \hline
%\# cells & \# dofs &
%\multicolumn{2}{|c|}{${L^2(0,T;\SSpace)}$} &
%\multicolumn{2}{|c|}{${L^{\infty}(0,T;L^2(\Omega))}$}\\ \hline
\multicolumn{6}{c}{${\tt m}\equiv 2$}\\ \hline
4 & 72 & 4.781e+00 & - & 3.812e-01 & -\\ \hline
16 & 288 & 1.013e+00 & 2.24 & 5.422e-02 & 2.81\\ \hline
64 & 1152 & 2.282e-01 & 2.15 & 7.330e-03 & 2.89\\ \hline
256 & 4608 & 5.480e-02 & 2.06 & 1.240e-03 & 2.56\\ \hline
1024 & 18432 & 1.349e-02 & 2.02 & 1.743e-04 & 2.83\\ \hline
4096 & 73728 & 3.427e-03 & 1.98 & 2.259e-05 & 2.95\\ \hline
\end{tabular}
\end{center}
\caption{Convergence test. Errors and convergence rates under uniform mesh refinement. 
A fixed time step of size $.5\times 10^{-3}$
was used.
Linear (above) and quadratic (below) dG in space discretizations.
}
\end{table}

{\bf Advection-dominated test.} With this numerical example we test the robustness of the method in the advection-dominated regime. 
%The problem specifications are as follows, {\em c.f.}~\eqref{pde}: 
We consider once again the domain $\Omega=[-1,1]^2$ subdivided into the  subdomains $\Omega^1$ and $\Omega^2$ already considered in the previous test. In $\Omega$, we solve a scalar equation with no reaction and the 
constant diffusion $a_1=10^{-2}$ 
and the advection field $B_1=(0.5,0.5)$. 
On the boundary $\partial\Omega$, we set homogeneous Neumann boundary conditions. 
\eqref{transmission}
 The parameters %constant and diagonal permeability tensor 
\[
\mbf{P}=2/10, 
\qquad 
\Weight^{1} =5/6,
\qquad 
\Weight^{2} =1/6,
\qquad 
\Friction =6/10,
\]
are used in the  interface conditions~\eqref{transmission}. Thus transfer across the interface is mainly advection-driven. Further, notice that setting a friction coefficient to
less than one models the case in which the interface acts as a filtering wall on the advected quantity; hence a boundary layer in the upwind subdomain in the proximity of the interface is expected. 

We solve the problem on a uniform $16\times 16$ mesh using linear elements. Such mesh is not fine enough to resolve the layer forming in the proximity of the interface where the solution is also discontinuous, see Figure~\ref{fig:ex2sol:16}. Nevertheless, the numerical solution is stable, and the expected behaviour of the solution is accurately captured, as we can see by comparison with the solution obtained with a layer resolving $64\times 64$ mesh and shown in Figure~\ref{fig:ex2sol:64}. 
\begin{figure}
\centering
\includegraphics[scale=0.12]{figures/ref4_sol_0_10_20_30_40_50_60_70.pdf}
\caption{Advection-dominated test. Snapshots of the solution computed on a uniform $16\times 16$ mesh using linear elements: the initial condition (top-left) followed by the solution at time intervals of $0.5$.}
\label{fig:ex2sol:16}
\end{figure}
\begin{figure}
\centering
\includegraphics[scale=0.2]{figures/ref6_sol_10_20.pdf}
\caption{Advection-dominated test. Snapshots of the solution computed on a uniform $64\times 64$ mesh using linear elements: solution at $t=0.5$ (left) and $t=1$ (right) corresponding to the second and third plots in the first row of Figure~\ref{fig:ex2sol:16}, respectively.}
\label{fig:ex2sol:64}
\end{figure}


%Other tests: %In particular we may want to test the theta term (question by Makridakis).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
